React-tRace: A Semantics for Understanding React Hooks

React has become the most widely used web front-end framework, enabling the creation of user interfaces in a declarative and compositional manner. Hooks are a set of APIs that manage side effects in function components in React. However, their semantics are often seen as opaque to developers, leading to UI bugs. We introduce React-tRace, a formalization of the semantics of the essence of React Hooks, providing a semantics that clarifies their behavior. We demonstrate that our model captures the behavior of React, by theoretically showing that it embodies essential properties of Hooks and empirically comparing our React-tRace-definitional interpreter against a test suite. Furthermore, we showcase a practical visualization tool based on the formalization to demonstrate how developers can better understand the semantics of Hooks.

==> acmart-preload-hook.tex <==
% Load before hyperref
\PassOptionsToPackage{dvipsnames}{xcolor}

% WARN: Remove before submission
% \PassOptionsToPackage{showframe}{geometry}
%\PassOptionsToPackage{draft}{graphicx}

